Cornucopia: A Framework for Feedback Guided Generation of Binaries

Binary analysis is an important capability required for many security and software engineering applications. Consequently, there are many binary analysis techniques and tools with varied capabilities. However, testing these tools requires a large, varied binary dataset with corresponding source-level information. In this paper, we present Cornucopia, an architecture agnostic automated framework that can generate a plethora of binaries from corresponding program source by exploiting compiler optimizations and feedback-guided learning. Our evaluation shows that Cornucopia was able to generate 309K binaries across four architectures (x86, x64, ARM, MIPS) with an average of 403 binaries for each program and outperforms Bintuner, a similar technique. Our experiments revealed issues with the LLVM optimization scheduler resulting in compiler crashes ($\sim$300). Our evaluation of four popular binary analysis tools Angr, Ghidra, Idapro, and Radare, using Cornucopia generated binaries, revealed various issues with these tools. Specifically, we found 263 crashes in Angr and one memory corruption issue in Idapro. Our differential testing on the analysis results revealed various semantic bugs in these tools. We also tested machine learning tools, Asmvec, Safe, and Debin, that claim to capture binary semantics and show that they perform poorly (For instance, Debin F1 score dropped to 12.9% from reported 63.1%) on Cornucopia generated binaries. In summary, our exhaustive evaluation shows that Cornucopia is an effective mechanism to generate binaries for testing binary analysis techniques effectively.

==> sections/OldDesign.tex <==
\section{Design}
\label{sec:Design}

The Design of ~\ourtool{} consist of various pieces working in harmony together to enable the generation of various variants from the source file. We now separate our discussion of the various phases as follows: Compiling sources, ~\AFL{} mutations, Post-processor Phase, Main binary, Fitness Function calculation and Server Response.
\newline
\textbf{TODO:} (ADD to the sections below for the GCC part)

\begin{itemize}
  \item \textit{Compiling sources}: We scrape multiple Debian sources and get .tar files for various sources. We then use an automated script that extracts these tart files, builds them using our own modified version of WLLVM (maybe add a macro for this, not sure of the name for the wllm tool that we have made?) and extracts bit-code files from all compiled binaries to get a collection of Debian sources for fuzzing. In addition we use rust sources from crates.io
  \item \textit{~\AFL{} mutations}: We use ~\AFL{} to mutate bytes and use those mutated bytes to prepare commands that we feed to the LLVM static compiler (LLC). The LLVM static compiler has approximately 800+ optimization options listed when we spill them using ``llc --help-hidden''. These optimization options are parsed using a program and written to a file. These commands will be further used for compiling source files by our post-processor. We modified ~\AFL{}'s scheduling policy to prioritize bytes on the queue in accordance with a weight parameter. This weight parameter is used internally by ~\AFL{} to determine which mutated byte string has the highest priority and further mutations are prioritized. That is, ~\AFL{} considers the path that led to the highest weighted mutated byte as the most interesting and prioritizes mutations to this path more than others. On the other hand, if the weight returned is 0, ~\AFL{} considers these paths as uninteresting and prunes the search accordingly.
  \item \textit{Post-processor phase}: The Post-Processor is a main component of the infrastructure, You can imagine it as the brain of the system. It parses the mutated bytes from ~\AFL{} and constructs a command that is used by the LLVM static compiler for compilation. The post-processor is written in C++, it reads all the available compilation commands from file and stores them in an internal buffer. Each byte in the mutated byte string sent by ~\AFL{} corresponds to a compilation option in our model. Since the value of a byte can range from 0-255, we use a modulus 2 operation on each bytes as a toggle to determine if we want to use an option or not. For instance, if ``byte mod 2 == 0'' we do not use that particular option, if its 1 then we do. This uniformly distributes weather a particular LLVM static compiler option is used or not. For options that require a (int, uint) value, we assign the value as (byteVal - 1) / 2. This makes sure that each odd number now results in a integer series from (0,1,2,...). 
  Using these constraints, the post-processor constructs an option string which is used to compile the source file using the LLVM static compiler. The post-processor performs correct error checking using the return code from LLC, if an error code is returned the post-processor instead compiles the -O0 version of the source file. The intution behind this is that since the over time ~\AFL{} will figure out that since all error compilations result in the O0 compile binary it will stop taking paths that result in the crashes. Further, depending on the fitness function, the .s file generated by LLC is further compiled to a binary using clang without any additional optimization options.
  \item \textit{Main binary}: The main binary is a C source file that is responsible for handshaking with the server and serving as an intermediary between the server and ~\AFL{}. You can think of this binary as the ``actual'' binary that is fuzzed my ~\AFL{}. Once the post-processor compiles the source into either a .s file or a binary, ~\AFL{} sends this binary to main binary. The main binary handshakes with the server, sends this binary to our server, get a response back (weight of this particular binary) and depending on the weight, the main tell  ~\AFL{} is the binary sent was interesting or not. If interesting, it also send ~\AFL{} the corresponding weight which is calculated using some fitness function heuristic.
  \item \textit{Fitness Function Calculation}: The fitness function calculation is integral to driving ~\AFL{} and in turn our tool to generate quality binaries. The fitness function calculates a score (weight) defining how important or qualitatively important the binary seen is. Using heuristics we determine a score for the binary against either the -O0 compiled version or all the binaries seen so far for that particular source file. We use metrics such as Normalized Compression Distance (NCD), SSDEEP, etc.. (discussed more in the fitness function section).
  \item \textit{Server Response}: Once the server receives the binary from the main binary, it checks to see if the binary is already present in a locally maintained database. If it is, the server doesn't add this binary to the database and return a 0 weight signalling ~\AFL{} that the current binary is uninteresting. On the other hand, if the binary is not seen in the database, the server calculates a score based on the fitness function chosen, add the binary to the database and send the calculated score to ~\AFL{} signalling ~\AFL{} to mark it interesting. Internally ~\AFL{} uses this weight in scheduling and finding more paths as discussed before.
\end{itemize}

To accelerate the process of generating new binaries from multiple sources, we parallelize ~\ourtool{} to run each source in parallel instead of sequentially running all sources. For now we parallelize at the level of the source file (we don't parallelize the instance of one particular soucrce file but run multiple ~\AFL{} instaces on different source files). In the future we have plans for a more advanced scheduling technique to make ~\ourtool{} more efficient.
Parallelizing at the source level results in an accelerated generation of binaries across all sources. In addition we support multiple architectures for LLVM by using gnu-multilib and other cross compilation packages on x86-64. We also have the capability to easily change the fitness function heuristic used. This can enable easy modifications and enable users to port their fitness function policy easily onto ~\ourtool{}. 

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Despite our aim to generate a large number of binaries,~\ourtool{} may not generate~\emph{all} possible binaries for a given source.
We are limited by the ability of the underlying compiler to produce different binaries.
Compilers aim to generate performance-efficient and straightforward binaries.
Consequently, general-purpose compilers do not support obfuscation-related program transformations, such as control-flow flattening~\cite{laszlo2009obfuscating} and VM-based obfuscation~\cite{fang2011multi}, which complicate the binary.

We want to emphasize that~\ourtool{}~\emph{does not} replace existing obfuscation-related techniques but rather complements them.
This work demonstrates an alternative, low-effort method to generate semantically equivalent binaries by using existing compilers.


==> sections/evaluationold.tex <==
\section{Evaluation}
\label{sec:evaluation}
We evaluate~\ourtool{} to demonstrate its effectiveness in generating semantically equivalent binaries and their ability to test the robustness of various binary analysis tools.
Specifically, we attempt to evaluate the following aspects:
\begin{itemize}
\item\textbf{Effectiveness:} How effective is~\ourtool{} in generating binaries, and how do different fitness metrics affect the quality and quantity of the generated binaries?
\item\textbf{Throughput:} What is the throughput of~\ourtool{} in generating binaries from a given source package?
\item\textbf{Robustness of static analysis tools:} How effective is the dataset generated by~\ourtool{} in revealing robustness issues in binary static analysis tools?
\item\textbf{Robustness of~\ac{ML} tools:} How effective is dataset generated by~\ourtool{} in revealing robustness issues in~\ac{ML} tools?
\end{itemize}

%RQ1: How different are the generated binaries w.r.t the default and other optimization levels.
%   - We will use our metric (hash based one) and the one use in BinTuner (i.e., BinHunt).
   
%RQ2: Throughput: How fast does our technique generate binaries. We should also compare different feedback mechanisms here.

%We use different fitness function metrics to generate a score that tells ~\AFL{} how important a variant is. We use a fitness function metric named "function hash" that generates an approximate of 180,000 variants for 500 source files in around 6 hours for the x86-64 architecture. 

%RQ3: How effective is our technique in exposing issues with binary analysis tools.

%RQ4: How effective is our technique in exposing issues with Machine learning models.

\subsection{Dataset and Compilers}
We choose~\clangversion{} (or LLVM) and~\gccversion{} as the target compilers.
They both are representative of two different compiler variations.
For~\code{clang} our binary generator is more efficient as it runs optimizers on the LLVM Bitcode avoiding frontend, whereas for~\code{gcc} we run the entire compiler pipeline, including its frontend.

For source packages, we scrapped official Debian package repositories and selected random~\numllvmpackages{} packages that we could compile using~\clangversion on an updated Ubuntu 20.04 machine with certain basic libraries installed.
Similarly, we selected another~\numgccpackages{} packages that we could compile using~\gccversion{}. We found certain packages that~\emph{failed} to compile using~\gccversion{}, hence the difference in the number of packages.

We chose~\xeightsix{},~\xsixfour{},~\arm{},and,~\mips{} architectures for~\clangversion{}, where as only~\xsixfour{} for~\gccversion{}.
The main reason for missing architectures for ~\gccversion{} is the difficulty in setting up a cross-compilation toolchain and building the dependencies for each of the architecture.
For~\clangversion{}, it was easy as we directly used bitcode file and used ~\code{--march=<arch>} and ~\code{-Wl,--unresolved-symbols=ignore-in-object-files} this avoided all errors because of the header file and linker dependencies.
Where as we could not find similar flags for~\gccversion{} as we were compiling from the sources.
We want to emphasize that these are not fundamental limitations of~\ourtool{} but rather build system dependencies that could be solved with some engineering effort of setting up cross-compilation toolchains.

\subsection{Effectiveness of fitness metrics}
We use different fitness function metrics to send feedback to ~\AFL{} , these metrics differ in the mechanism in which they calculate the weight (importance) to give to a particular variant of that source file.
We briefly discuss the various fitness function metrics we use to generate variants for each source file and compare the effectiveness of each fitness function metric with each other. 
\newline
We use NCD (Normalized Compression Distance) which is also used by Ren et al.~\cite{ren2021unleashing} which is an information theory metric useful to calculate the similarity between sequences of bytes. We use lzma compression to compress the binaries similar to Ren et al. We calculate a floating point score between 0 and 1, 0 being no difference and 1 being completely different and send that as a feedback to ~\AFL{}. We develop three different algorithms which are variations on NCD and are discussed below.  
    \begin{itemize}
        \item {\textit{NCD original}: We use NCD (Normalized Compression Distance) to always compare the new variant seen with the -O0 compiled binary of the source code. The NCD computation now gives us a score between 0 and 1. (0 corresponds to completely identical binaries and 1 to completely different binaries) This is similar to how Ren et al. compute the score for each new binary that they see in their framework.}
        \item {\textit{NCD average}: We use take a running average of the NCD scores amongst the new variant with all variants that are already in the database for that particular source file. The intuition behind using a running average is that it will converge slowly (intuitively providing ~\AFL{} to potentially find more variants, by figuring out more paths) and provide a measure of relative difference across all variants rather that just measuring the weight against the -O0 compiled binary.}
        \item {\textit{NCD min}}: We use NCD to calculate the weight of the new variant with all the existing binaries that are already in the database. We then send the minimum score from that pool as feedback to ~\AFL{}. The intuition behind sending the minimum is similar to that of the average metric in that we want to explore the weight across all the variants rather than just compare against the -O0 compiled binary. However, using the min offers faster convergence than the average case which might help speedup our framework and help it get out of local minimums faster if stuck at one.
    \end{itemize}
    ssdeep is a program to compute context triggered piecewise hashes (fuzzy hashes). ssdeep is designed to figure out input strings that have homologies. Homologies are strings that have sequences of bytes in the same order. We want to test the effectiveness of ssdeep as a function of testing the difference between binaries. ssdeep returns a score of 100 if the binaries are completely similar and 0 if they are completely different. We invert this score by subtracting it from 100 and normalize it which is then send back to ~\AFL{} as feedback.
    \begin{itemize}
        \item {\textit{ssdeep average}:  We use ssdeep.hash to hash the new variant of the binary using its .text section. We get a score between 0 and 100 by using ssdeep.compare across. We invert and normalize this score and take an average of all the ssdeep scores for the new variant against each binary that is already in the database. This score is then returned by the server to ~\AFL{}. The intuition behind using the average is similar to the NCD average case where want to test the difference across all the variants rather than just the -O0 compiled binary and also converge slowly so that ~\AFL{} can find more paths.}
        \item {\textit{ssdeep min}}: We use ssdeep.hash to hash the new variant of the binary using its .text section and get a score between 0 and 100 similar to the average case. But instead of returning the average of the scores for all the variants we return the min score. We expect the min to converge more quickly than the average which may get us out of local minimums faster than the average case.
    \end{itemize}
We use of own metric named as "Function Hash". The "Function Hash" technique is implemented in the LLVM \textit{ASMPrinter}. We generate a hash for each function by using std::hash on the function body. At the same time, we maintain a global hash for a variant that is a generated by sorting all the function hashes to get rid of any ordering differences in functions and finally taking a hash of the sorted vector of function hashes. We make use of this global hash to determine the uniqueness of the generated binary. In addition, we send a weight to ~\AFL{} as feedback which is the sum of all new functions seen across all the variants currently in the database for that particular source normalized by the total number of functions in the variant. In short, this metric tells us "the percentage of unique functions in the current variant".

To evaluate and compare the effectiveness of the fitness functions, we conduct multiple experiments. As mentioned before, we modify ~\AFL{} so that it does its internal scheduling based using an additional weight parameter, that sorts the command bytes based on their relative weight. ~\AFL{} still chooses the bytes randomly but now this random picking is weighted. Bytes with higher weigh are more likely to be explored first. We test the effectiveness of our fitness functions with two different \AFL{} versions. One with the weight parameter enabled and one where the weight parameter is disabled. In addition, we noticed that ~\AFL{} uses a different seed value for different instances and this will cause the performance of the fitness function to be random. Since ~\AFL{} may take different paths at different instances due to the randomness instilled in ~\AFL{}. For this reason for each fitness function we ran multiple instance in order to get a sense of how well that fitness function performs relative to other fitness functions.
We saw that our "function hash" technique is able to find the highest number of variants for a source file for a fixed amount of time. In addition we can be sure that these variants are "true positives" since we compare the differences in function body only and also get rid of any ordering differences. Our implementation if fast and offers advantage against NCD and ssdeep which may take more computation time due to compression etc. We also noticed that our weighted branch of ~\AFL{} produced more binaries that the non-weighted branch for a fixed amount of time. Which makes sense because the higher weighted binaries will lead to greater paths than the less weighted binaries.

The "function hash" technique is aimed to find the differences in functions across all the variants for that particular source file and not just the -O0 compiled variant.

% \begin{table}[h!]
% \centering
% \begin{tabular}{ |p{2.5cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}| } 
% \hline
% fitness function & WI & WT & NWI & NWT \\
% \hline
% \multirow{6}{*}{}NCD average &  &  &  &  \\ 
% \hline
% NCD min &  &  &  &  \\
% \hline
% NCD original &  &  &  &  \\ 
% \hline
% SSDEEP average &  &  &  &  \\
% \hline
% SSDEEP min &  &  &  &  \\ 
% \hline
% function hash &  &  &  &  \\ 
% \theAlgoLine{}
% \end{tabular}
% \caption{This table shows the performance of different fitness functions. W = weighted, N = Not, I = Iterations, T = Time}
% \end{table}

\subsection{Impact on Binary Similarity}
We use BinHunt to compare the similarity of the 
generated binaries with different optimization flags.

\input{figures/through}

\input{figures/variations}

\subsection{Robustness testing of Static Binary Analysis tools}
what binary analysis tools we use, setup and how we test each tool.
IDA, GHIDRA, angr, radare2

What analysis we should run?

angr - Function boundaries.

Calling convention analysis - differential analysis.

IDA - get calling convention call.
Ghidra - get calling convention call.

\subsection{Robustness testing of Machine Learning techniques}
Debug information: Debin.

Binary similarity (these are the tools used in BinTuner as well): Asm2Vec, INNEREYE, and DeepBinDiff.


==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivaton}
Why we need this? What is the need of such a system? Do we have evidence of a problem that our system might help with?

Binary analysis frameworks are generally tested on binaries that are compiled using standard optimization options like O3, O2..etc. Although these options in itself perform many optimization passes under the hood, we argue that these standard optimization options do not cover the full range of optimization options that are available in compiler toolchains like LLVM and GCC. Binary analysis tools are not thoroughly tested on these "variants" of the standard binaries and therefore offer a way to find vulnerabilities in these binary analysis tools. In addition a recent paper bintuner showed how viruses metamorphosize using additional available optimization options other than standard Ox options; binary difference tools like "binhunt "and "bindiff" did poorly in identifying these variants. ~\ourtool{} can help in the development of more robust binary analysis tools by maximizing the generation of these variants and providing a Corpus of binaries that can be tested upon by binary analysis tools
...continue

==> tables/bintoolcrash.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|r|r|r|r}
\toprule
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}r@{}}Tool$\rightarrow$\\ $\downarrow$Architecture\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\angr}} & \multicolumn{1}{c|}{\textbf{\ghidra}} & \multicolumn{1}{c|}{\textbf{\idapro}} & \multicolumn{1}{c}{\textbf{\radare}} \\ 
\midrule

\rowcolor{black!15} {\xeightsix}                                                                               &       107                    &     0                  &  0                                 &  0                                \\ 

{\xsixfour}                                                                               &                  81               &         0                             &            0                       &   0                               \\ 

\rowcolor{black!15} {\arm}                                                                               &         21                         &              0                       &               1                   &        0                        \\

{\mips}                                                                              &                   6                 &                   0                   &                  0                 &                    0              \\
%{\xsixfour gcc}                                                                              &                   48                 &                   0                   &                  0                 &                    0              \\

\midrule
\rowcolor{black!15} \textbf{Total}                                                                             &            263                    &          0                            &         1                         &          0                        \\ 
\bottomrule
\end{tabular}
\caption{Number of randomly sampled binaries that resulted in failures (crashes or graceful failure with empty result) of the corresponding tools.}
\label{tab:toolcrash}
\end{table}


==> tables/bintooldiff.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c||rr||rr||rr}
\toprule
\multirow{2}{*}{\textbf{Architecture}} & \multicolumn{2}{c||}{\textbf{Function Boundary Detection}}              & \multicolumn{2}{c||}{\textbf{Calling Convention Recovery}}              & \multicolumn{2}{c}{\textbf{Control Flow Graph Recovery}}              \\ \cline{2-7} 
                                       & \multicolumn{1}{c|}{\textbf{\failures}} & \multicolumn{1}{c||}{\textbf{\failurem}} & \multicolumn{1}{c|}{\textbf{\failures}} & \multicolumn{1}{c||}{\textbf{\failurem}} & \multicolumn{1}{c|}{\textbf{\failures}} & \multicolumn{1}{c}{\textbf{\failurem}} \\ 
                                       \midrule
\rowcolor{black!15} \textbf{\xeightsix}      & \multicolumn{1}{r|}{13143}  &   2733   & \multicolumn{1}{r|}{12494}   &  191     & \multicolumn{1}{r|}{15696}    &      138  \\ 
\textbf{\xsixfour}                           & \multicolumn{1}{r|}{429}    &   106    & \multicolumn{1}{r|}{417}     &  31      & \multicolumn{1}{r|}{764}      &       17   \\ 
\rowcolor{black!15} \textbf{\arm}            & \multicolumn{1}{r|}{923}    &   132    & \multicolumn{1}{r|}{56}      &  18      & \multicolumn{1}{r|}{137}      &       82   \\ 
\textbf{\mips}                               & \multicolumn{1}{r|}{6869}   &   20292  & \multicolumn{1}{r|}{20931}   &  3510    & \multicolumn{1}{r|}{30163}    &     5643   \\ 
\midrule

\rowcolor{black!15} \textbf{Total}          & \multicolumn{1}{r|}{21364}   &   23263  & \multicolumn{1}{r|}{33898}   &  3750    & \multicolumn{1}{r|}{46760}    &     5880   \\ 
\bottomrule
\end{tabular}
\caption{Results of differential testing of various analysis using. Here,~\failures and~\failurem indicate the number of binaries with single tool divergence (\ie only one tool produces a different result) and multi-tool divergence (\ie Multiple tools produce different results), respectively.}
\label{tab:tooldifftesting}
\end{table*}


==> tables/bintooldiffnew.tex <==
{

\begin{table*}[]
\centering
\fontsize{6pt}{6pt}\selectfont
\begin{tabular}{c|r||rrrr|r||rrrr|r||rrrr|r}

\toprule
\multirow{3}{*}{\textbf{Arch.}} & \multicolumn{1}{c||}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Randomly} \\ \textbf{Sampled} \\ \textbf{Binaries}\end{tabular}}} & \multicolumn{5}{c||}{\textbf{Function Boundary Detection}}                                                                                                                                                           & \multicolumn{5}{c||}{\textbf{Calling Convention Recovery}}                                                                                                                                                           & \multicolumn{5}{c}{\textbf{Control Flow Graph Recovery}}                                                                                                                                                           \\ \cline{3-17} 
                              & \multicolumn{1}{c||}{}                                                                           & \multicolumn{4}{c|}{\textbf{\failures}}                                                                                  & \multicolumn{1}{c||}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\failurem}\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\failures}}                                                                                  & \multicolumn{1}{c||}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\failurem}\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\failures}}                                                                                  & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\failurem}\end{tabular}}} \\ \cline{3-6} \cline{8-11} \cline{13-16}
                              & \multicolumn{1}{c||}{}                                                                           & \multicolumn{1}{c}{\angr} & \multicolumn{1}{c}{\ghidra} & \multicolumn{1}{c}{\idapro} & \multicolumn{1}{c|}{\radare} & \multicolumn{1}{c||}{}                                                                       & \multicolumn{1}{c}{\angr} & \multicolumn{1}{c}{\ghidra} & \multicolumn{1}{c}{\idapro} & \multicolumn{1}{c|}{\radare} & \multicolumn{1}{c||}{}                                                                       & \multicolumn{1}{c}{\angr} & \multicolumn{1}{c}{\ghidra} & \multicolumn{1}{c}{\idapro} & \multicolumn{1}{c|}{\radare} & \multicolumn{1}{c}{}                                                                       \\ \midrule

                              
                              
                              \rowcolor{black!15} {\xeightsix clang}                           &                                        8524                                                         & \multicolumn{1}{r|}{715}      & \multicolumn{1}{r|}{821}       & \multicolumn{1}{r|}{2200}    & \multicolumn{1}{r|}{8492}   &            2483                                                                                 & \multicolumn{1}{r|}{98}     & \multicolumn{1}{r|}{39}       & \multicolumn{1}{r|}{6101}    & \multicolumn{1}{r|}{4035}   &                                      7615                                                       & \multicolumn{1}{r|}{2992}     & \multicolumn{1}{r|}{161}       & \multicolumn{1}{r|}{227}    & \multicolumn{1}{r|}{4671}   &                                       8230                                                      \\ 

                              
                              {\xsixfour clang}                           &                                                  3516                                               & \multicolumn{1}{r|}{213}     & \multicolumn{1}{r|}{302}       & \multicolumn{1}{r|}{255}    & \multicolumn{1}{r|}{2349}   &                                     563                                                        
                              & \multicolumn{1}{r|}{901}     & \multicolumn{1}{r|}{260}       & \multicolumn{1}{r|}{2184}    & \multicolumn{1}{r|}{2105}   &          2386                                                                              & \multicolumn{1}{r|}{1214}     & \multicolumn{1}{r|}{115}       & \multicolumn{1}{r|}{745}    & \multicolumn{1}{r|}{1915}   &                                   3015                                                          \\ 

                              
                              \rowcolor{black!15} {\arm clang}                           &                           5382                                                                      & \multicolumn{1}{r|}{2388}     & \multicolumn{1}{r|}{2891}       & \multicolumn{1}{r|}{2872}    & \multicolumn{1}{r|}{3324}   &                      3020                                                                       & \multicolumn{1}{r|}{2975}     & \multicolumn{1}{r|}{420}       & \multicolumn{1}{r|}{2769}    & \multicolumn{1}{r|}{2893}   &                                     3990                                                        & \multicolumn{1}{r|}{1722}     & \multicolumn{1}{r|}{84}       & \multicolumn{1}{r|}{61}    & \multicolumn{1}{r|}{2354}   &                   5222                                                          \\ 

                              
                              {\mips clang}                          &                                4818                                                                 & \multicolumn{1}{r|}{2744}     & \multicolumn{1}{r|}{2149}       & \multicolumn{1}{r|}{679}    & \multicolumn{1}{r|}{3750}   &                                 2977                                                            & \multicolumn{1}{r|}{522}     & \multicolumn{1}{r|}{122}       & \multicolumn{1}{r|}{1166}    & \multicolumn{1}{r|}{2705}   &                 4126
                              & \multicolumn{1}{r|}{1968}     & \multicolumn{1}{r|}{23}       & \multicolumn{1}{r|}{40}    & \multicolumn{1}{r|}{1514}   &                                            4583                                                 \\

                              
                              \rowcolor{black!15}{\xsixfour gcc}                          &                                1554                                                                 & \multicolumn{1}{r|}{1}     & \multicolumn{1}{r|}{1}       & \multicolumn{1}{r|}{290}    & \multicolumn{1}{r|}{1218}   &                                 286                                                            
                              & \multicolumn{1}{r|}{953}     & \multicolumn{1}{r|}{9}       & \multicolumn{1}{r|}{1060}    & \multicolumn{1}{r|}{997}   &       1239                                                                           & \multicolumn{1}{r|}{214}     & \multicolumn{1}{r|}{34}       & \multicolumn{1}{r|}{161}    & \multicolumn{1}{r|}{1006}   &                                            1230                                                 \\ \midrule

 
 
 
 \textbf{Total}                         &                                         23794                                                        & \multicolumn{1}{r|}{6061}     & \multicolumn{1}{r|}{6164}       & \multicolumn{1}{r|}{6296}    & \multicolumn{1}{r|}{19133}   &                                9329                                                             & \multicolumn{1}{r|}{5449}     & \multicolumn{1}{r|}{850}       & \multicolumn{1}{r|}{13280}    & \multicolumn{1}{r|}{12735}   &                                            19356                                                 & \multicolumn{1}{r|}{8110}     & \multicolumn{1}{r|}{417}       & \multicolumn{1}{r|}{764}    & \multicolumn{1}{r|}{11460}   &                                        22280                                                     \\ 
\bottomrule
\end{tabular}
\caption{Results of differential testing of various analysis using. Here,~\failures and~\failurem indicate the number of binaries with single tool divergence (\ie only one tool produces a different result) and multi-tool divergence (\ie Multiple tools produce different results), respectively.}
\label{tab:tooldifftesting}
\end{table*}
}


==> tables/mltooldiff.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{c||rr||rr||r}
% \toprule
% \multicolumn{1}{c||}{\multirow{2}{*}{\textbf{Architecture}}} & \multicolumn{2}{c||}{\textbf{\asmvec}}                                          & \multicolumn{2}{c||}{\textbf{\debin}}                                             & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Difference\end{tabular}}}} \\ \cline{2-5}
% \multicolumn{1}{c||}{}                                       & \multicolumn{1}{c|}{\textbf{Reported}} & \multicolumn{1}{c||}{\textbf{Observed}} & \multicolumn{1}{c|}{\textbf{Reported}} & \multicolumn{1}{c||}{\textbf{Observed}} & \multicolumn{1}{c|}{}                                                                                        \\ \midrule
% \rowcolor{black!15}\textbf{\xeightsix}        &        &       &       63.1        &    12.89      &                   \\
% \xsixfour                                     &        &       &       68.6        &    18.19      &                   \\
% \rowcolor{black!15}\textbf{\arm}              &        &       &       64.5        &    13.6       &                   \\
% \mips                                         &        &       &                   &               &                   \\
% \midrule
% \rowcolor{black!15}\textbf{Average}           &        &       &                   &               &                    \\
% \bottomrule
% 
% \end{tabular}
% \caption{Robustness of~\ac{ML} tools: The columns~\textbf{Reported} and~\textbf{Observed} show the precision reported in the corresponding paper and precision observed when tested with the binaries generated by~\ourtool.}
% \label{tab:mltooldifftesting}
% \end{table*}


==> tables/programsArchitecture.tex <==
\begin{table}[h]
\centering
\begin{tabular}{ c|c|c } 
\toprule
\textbf{Architecture} & \textbf{No. of Programs} & \textbf{Compiler Options} \\
\hline
\rowcolor{black!15} \multirow{3}{0em}{}x86 clang & 191   &  892 \\
x64 clang & 191 & 892 \\ 
\rowcolor{black!15} ARM clang & 191  &  876  \\ 
MIPS clang & 191 & 866  \\
\rowcolor{black!15} x64 gcc & 307  &  255  \\
\bottomrule
\end{tabular}
\caption{Number of programs used for binary generation for each architecure and compiler configuration.}
\label{tab:programsArch}
\end{table}


==> tables/variationstabold.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|r|rrr}
\toprule
\textbf{Architecture} & \multicolumn{1}{l|}{\textbf{Binaries}} & \multicolumn{1}{l|}{\textbf{Programs}} & \multicolumn{1}{l|}{\textbf{Flags}} & \multicolumn{1}{l}{\textbf{Avg. variants}} \\ 
\midrule
\rowcolor{black!15} {\xeightsix clang}  &   63197  &   \multicolumn{1}{r|}{191} &   \multicolumn{1}{r|}{892}   & \multicolumn{1}{r}{330.87}   \\  
{\xsixfour clang}                       &   74169  &   \multicolumn{1}{r|}{191} &   \multicolumn{1}{r|}{892}   & \multicolumn{1}{r}{388.32}   \\ 
\rowcolor{black!15} {\arm clang}        &   83701  &   \multicolumn{1}{r|}{191} &   \multicolumn{1}{r|}{876}   & \multicolumn{1}{r}{438.23}   \\ 
{\mips clang}                           &   87192  &   \multicolumn{1}{r|}{191} &   \multicolumn{1}{r|}{866}   & \multicolumn{1}{r}{456.50}   \\ 
\rowcolor{black!15}{\xsixfour gcc}      &   1554   &   \multicolumn{1}{r|}{307} &   \multicolumn{1}{r|}{255}   & \multicolumn{1}{r}{5.32}     \\ 
\midrule\textbf{Grand Total}            &   309813 &   \multicolumn{3}{c}{N/A}                                                                 \\ 
\bottomrule
\end{tabular}
}
\caption{Performance of~\clangversion{} and~\gccversion{} across various architectures.}
\label{tab:variationsarchclang}
\end{table}
